Explaining Black Box Predictions and Unveiling Data Artifacts through Influence Functions

Modern deep learning models for NLP are notoriously opaque. This has motivated the development of methods for interpreting such models, e.g., via gradient-based saliency maps or the visualization of attention weights. Such approaches aim to provide explanations for a particular model prediction by highlighting important words in the corresponding input text. While this might be useful for tasks where decisions are explicitly influenced by individual tokens in the input, we suspect that such highlighting is not suitable for tasks where model decisions should be driven by more complex reasoning. In this work, we investigate the use of influence functions for NLP, providing an alternative approach to interpreting neural text classifiers. Influence functions explain the decisions of a model by identifying influential training examples. Despite the promise of this approach, influence functions have not yet been extensively evaluated in the context of NLP, a gap addressed by this work. We conduct a comparison between influence functions and common word-saliency methods on representative tasks. As suspected, we find that influence functions are particularly useful for natural language inference, a task in which 'saliency maps' may not have clear interpretation. Furthermore, we develop a new quantitative measure based on influence functions that can reveal artifacts in training data.

==> resources/SA_across_models.tex <==
\begin{table}
    \centering
    \begin{tabular}{@{}lrr@{}}
    \toprule
     & Saliency & Influence\\
      \midrule
      BERT vs. BERT-linear & $28.30\%$ & $25.72\%$\\
      BERT vs. LSTM & $18.63\%$ & $20.05\%$\\
      BERT-linear vs. LSTM & $17.04\%$ & $6.91\%$\\
      \bottomrule
    \end{tabular}
    \caption{\sout{Average \textbf{overlap rate} of the top 10\% interpretation results given by saliency map (tokens) or influence function (training examples) on two different models.}}
    \label{tab:SA_across_models}
\end{table}

==> resources/SA_direct_consistency.tex <==
\begin{table}[h]
\small
\begin{center}
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{p{0.10\textwidth}rrrr}
    \toprule
    {Token saliency} & @10\% & @20\% & @50\% & @full\\
    \midrule
    {Lowest} & 1.306 & 0.823 & 0.366 & 0.216\\
    & $\pm 0.036$ & $\pm 0.022$ & $\pm 0.011$ & $\pm 0.009$\\
    {Median} & 1.312 & 0.828 & 0.392 & 0.210\\
    & $\pm 0.016$ & $\pm 0.010$ & $\pm 0.005$ & $\pm 0.004$\\
    {Highest} & 1.433 & 0.891 & 0.431 & 0.236\\
    & $\pm 0.041$ & $\pm 0.026$ & $\pm 0.013$ & $\pm 0.009$\\
    \bottomrule
\end{tabular} 
\end{center}
\caption{
Average \textbf{influence score} of top training examples that contain a token in test example with lowest, median, or highest saliency.
}
\label{tab:SA_direct_consistency}
\end{table}

==> resources/SA_example.tex <==
% \begin{table}[h]
% \small
% \begin{center}
% \renewcommand{\arraystretch}{1.3}
% \begin{tabular}{p{0.34\textwidth}r}
%     \toprule
%     \textbf{Test input}\\
%     {Seldom has a movie so closely matched the \uline{\textcolor{cyan}{spirit}} of a man and his work.} & \{positive\}\\
%     \midrule
%     \textbf{Most \uline{\textcolor{cyan}{influential}} training examples}\\
%     {Had more to do with imagination than market research.} & [positive]\\
%     {Thought that the German film industry can not make a delightful comedy centering on food.} & [positive]\\
%     {Knockaround Guys rarely seems interested in kicking around a raison d'etre that's as fresh-faced as its young-guns cast.} & [positive]\\
%     \bottomrule
% \end{tabular} 
% \end{center}
% \caption{
% \sout{Correctly predicted positive example.}
% }
% \label{tab:SA_qual_example_1}
% \end{table}



% \begin{table}[h]
% \small
% \begin{center}
% \renewcommand{\arraystretch}{1.3}
% \begin{tabular}{p{0.34\textwidth}r}
%     \toprule
%     \textbf{Test input}\\
%     {It's slow -- very, very \uline{\textcolor{cyan}{slow}}.} & \{negative\}\\
%     \midrule
%     \textbf{Most \uline{\textcolor{cyan}{influential}} training examples}\\
%     {Slow.} & [negative]\\
%     {Freaking out.} & [negative]\\
%     {Loses.} & [negative]\\
%     \bottomrule
% \end{tabular} 
% \end{center}
% \caption{
% \sout{Correctly predicted negative example.}
% }
% \label{tab:SA_qual_example_2}
% \end{table}



\begin{table}[h]
\small
\begin{center}
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{p{0.34\textwidth}r}
    \toprule
    \textbf{Test input}\\
    {A \uline{\textcolor{cyan}{sometimes}} \uwave{\textcolor{red}{tedious}} film.} & \{positive\}\\
    \midrule
    \textbf{Most \uline{\textcolor{cyan}{supporting}} training examples}\\
    {That is the recording industry in the current climate of mergers and downsizing.} & [positive]\\
    {Credulous.} & [positive]\\
    {An admittedly middling film.} & [positive]\\
    \midrule
    \textbf{Most \uwave{\textcolor{red}{opposing}} training examples}\\
    {Full of cheesy dialogue.} & [negative]\\
    {Visually flashy but narratively opaque.} & [negative]\\
    {Luridly graphic.} & [negative]\\
    \bottomrule
\end{tabular} 
\end{center}
\caption{
An example in sentiment analysis interpreted by gradient-based saliency map and influence function.
}
\label{tab:SA_qual_example_3}
\end{table}



\begin{table}[h]
\small
\begin{center}
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{p{0.34\textwidth}r}
    \toprule
    \textbf{Test input}\\
    {Holden Caulfield \uline{\textcolor{cyan}{did}} it \uwave{\textcolor{red}{better}}.} & \{positive\}\\
    \midrule
    \textbf{Most \uline{\textcolor{cyan}{supporting}} training examples}\\
    {Better effects, better acting and a hilarious Kenneth Branagh.} & [positive]\\
    {Was better.} & [positive]\\
    {Much better.} & [positive]\\
    \midrule
    \textbf{Most \uwave{\textcolor{red}{opposing}} training examples}\\
    {Ticks off Kahlo's lifetime milestones with the dutiful precision of a tax accountant.} & [negative]\\
    {Its amiable jerking.} & [negative]\\
    {Come close to the level of intelligence and visual splendor that can be seen in other films.} & [negative]\\
    \bottomrule
\end{tabular} 
\end{center}
\caption{
\textbf{ALTERNATIVE} An example in sentiment analysis interpreted by gradient-based saliency map and influence function.
}
\label{tab:SA_qual_example_4}
\end{table}
